Sound and Complete Neural Network Repair with Minimality and Locality Guarantees

We present a novel methodology for repairing neural networks that use ReLU activation functions. Unlike existing methods that rely on modifying the weights of a neural network which can induce a global change in the function space, our approach applies only a localized change in the function space while still guaranteeing the removal of the buggy behavior. By leveraging the piecewise linear nature of ReLU networks, our approach can efficiently construct a patch network tailored to the linear region where the buggy input resides, which when combined with the original network, provably corrects the behavior on the buggy input. Our method is both sound and complete -- the repaired network is guaranteed to fix the buggy input, and a patch is guaranteed to be found for any buggy input. Moreover, our approach preserves the continuous piecewise linear nature of ReLU networks, automatically generalizes the repair to all the points including other undetected buggy inputs inside the repair region, is minimal in terms of changes in the function space, and guarantees that outputs on inputs away from the repair region are unaltered. On several benchmarks, we show that our approach significantly outperforms existing methods in terms of locality and limiting negative side effects. Our code is available on GitHub: https://github.com/BU-DEPEND-Lab/REASSURE.

==> Sections/recycle.tex <==
% \section{Appendix}\label{apx}
%     \begin{assumption}\label{asm: full rank}
%         We ask the $\Phi_{out}$ be $\{y| q_l\leq Py\leq q_u\}$ where $P$ is a full row rank matrix and $-\infty\leq q_l[i]\leq q_u[i]\leq +\infty$ ($q_l[i]$ and $q_u[i]$ is the i-th element of $q_l$ and $q_u$, respectively).
%     \end{assumption}
    
%     Remark: for most properties, they can be converted into this form, i.e, the classification problem in example \ref{exp: classification problem}.
    
%     We consider the following programming:
    
%     \begin{eqnarray}\label{eqn: linear transformation}
%         \begin{cases}
%         \min_T \max_{x\in A} |T(f(x) - f(x)|\\
%         T: R^{D_{out}} \to R^{D_{out}} \textit{ linear transformation}\\
%         q_l \leq P(T(f(A)))\leq q_u
%         \end{cases}
%     \end{eqnarray}
    
%     where $T$ is a linear transformation on neural network output space $R^{D_{out}}$. 
    
%     \begin{lemma}
%         We note $f(x) = f_1 x + f_2$. Assume $f_1$ is full rank, then we have programming \ref{eqn: linear patch function} and programming \ref{eqn: linear transformation} are equivalent.
%     \end{lemma}
    
%     \begin{proof}
%         On one side, for any $c, d$, since $f_1$ is full rank, there exists a transformation $T$, such that $T(f(x)) = T(f_1x+f_2) = (f_1+c)x + (f_2+d) = f(x) + cx + d$. 
        
%         On the other side, for any $T$, since $T(f(x)) - f(x)$ is a linear function, there exists $c, d$, such that $cx + d = T(f(x)) - f(x)$.
%     \end{proof}
    
%     Remark: for neural networks that are trained by a stochastic method, the probability $f_1$ is not full rank is 0.
    
%     To solve programming \ref{eqn: linear transformation}, for every row of $P$, say $i$-th row, we check the lower bound and upper bound of $P(f(A))$ by solving the following linear programming:
    
%     \begin{eqnarray}\label{LP: i-th row}
%         lb[i] = \min_{x\in A} P[i](f(A)) \\
%         ub[i] = \max_{x\in A} P[i](f(A)) 
%     \end{eqnarray}
    
%     where $P[i]$ is the $i$-th row of $P$. And find the minimal linear transform on $\mathbb{R}$ to move $[lb[i]. ub[i]]$ into $[q_l[i], q_u[i]]$.
    
%     Once we have linear transforms for every row, we can make it to a single linear transform $T$ on neural network output space $R^{D_{out}}$.
    
    % For most neural network, the output dimension is very low. We note all the vertex of $f(A)\subset Y$ to be $V(f(A))$. 
    
    % Therefore, \ref{eqn: linear transformation} becomes a linear programming if we consider $L_1$ or $L_\infty$ norm. It becomes a quadratic programming if we consider $L_2$ norm:
    
    % \begin{eqnarray}
    %     & \min_{T} \max_{v\in V(f(A))} |T(f(v)) - f(v)|\\
    %     & T(f(v)) \in \Phi_{out} \textit{ for all } v\in V(f(A))
    % \end{eqnarray}
    
    % In a special case, where $\Phi_{out} = [lb, ub]$ is an interval. And we note $f(x) = f_1x+f_2$ on linear region $A$.
    
    % We assume $cx = \alpha f_1 x$, where $\alpha\in R$ is undetermined coefficient, that is to say the linear patch function is parallel to neural network on $A$. We claim there exist $\alpha\in R$ and $d\in R$, such that the repair is both guaranteed and minimum.
    
    % We first find the minimum value $f_{min}$ and maximum value $f_{max}$ of $f(x) = f_1x$ for $x \in A$. 
    
    % \begin{enumerate}
    %     \item If $f_{max}-f_{min}\leq ub-lb$, we simply take $\alpha=0$ and $d = \min\{lb-f_{min}-f_2, ub-f_{max}-f_2\}$;
    %     \item If $max(f)-min(f) > ub-lb$, we simply take $\alpha=\frac{ub-lb}{max(f)-min(f)} - 1$ and $d = \frac{ub-lb}{max(f)-min(f)}min(f)-lb$. 
    % \end{enumerate}
    
    % In both case, our repair is guaranteed and minimum. We will show this in theorem \ref{thm: minimum repair}.

==> Sections/symbols.tex <==
        \begin{enumerate}
            \item $\Phi = (\Phi_{in}, \Phi_{out})$: the correctness specification, which requires $\forall x \in \Phi_{in}, f(x)\in \Phi_{out}$.
            \item $f$: the target DNN;
            \item $[0, 1]^m$: the input space for $f$ (here we assume all the data is normalized);
            \item $\mathbb{R}^n$: the output space for $f$;
            \item $\sigma$: ReLU activation function;
            \item $x$: an input of $f$;
            \item $z^i_j$: the $i^{\text{th}}$ hidden layer $j^{\text{th}}$ neuron value before activation function; $\hat{z}^i_j$: the $i^{\text{th}}$ hidden layer $j^{\text{th}}$ neuron value after activation function; 
            \item $\patcharea = \{x|Ax\leq b\}$: the patch area which is a linear region of target DNN $f$;
            \item $g_A(x, \gamma)$: the support network for $\patcharea$, which is similar to the characteristic function of $\patcharea$;
            \item $\gamma$: a parameter to control the side effect for patch;
            \item $p_A(x) = cx+d$: affine patch function, to guarantee the pre-given property;
            \item $h_A(x, \gamma)$: local patch network which is a combination of $p(x)$ and $g_A(x, \gamma)$;
            \item $\widehat{f}(x) = f(x) + h(x, \gamma)$: the repaired DNN;
            \item $\patcharea_i$ is the $i^{\text{th}}$ linear region needs to be repaired in the multiple patch case. $L$ is the total number of linear regions that needs to be repaired.
        \end{enumerate}
